Mesh2Tex: Generating Mesh Textures from Image Queries

Remarkable advances have been achieved recently in learning neural representations that characterize object geometry, while generating textured objects suitable for downstream applications and 3D rendering remains at an early stage. In particular, reconstructing textured geometry from images of real objects is a significant challenge -- reconstructed geometry is often inexact, making realistic texturing a significant challenge. We present Mesh2Tex, which learns a realistic object texture manifold from uncorrelated collections of 3D object geometry and photorealistic RGB images, by leveraging a hybrid mesh-neural-field texture representation. Our texture representation enables compact encoding of high-resolution textures as a neural field in the barycentric coordinate system of the mesh faces. The learned texture manifold enables effective navigation to generate an object texture for a given 3D object geometry that matches to an input RGB image, which maintains robustness even under challenging real-world scenarios where the mesh geometry approximates an inexact match to the underlying geometry in the RGB image. Mesh2Tex can effectively generate realistic object textures for an object mesh to match real images observations towards digitization of real environments, significantly improving over previous state of the art.

==> sections/tables.tex <==
\begin{table}[tp]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|l|cc|cc}
\toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{Parameterization} & \multicolumn{2}{c|}{Chairs} & \multicolumn{2}{c}{Cars} \\
% \midrule
    & & FID & KID \times $10^2$ & FID & KID \times $10^2$ \\
\midrule
    EG3D & Tri-plane Implicit & 36.45 & 2.15 & 83.11 & 5.95 \\
    Yu et al. & UV & 38.98 & 2.46 & 73.63 & 5.77 \\
    GET3D & Tri-plane Implicit & \ \ 46.20^* & \ \ 3.02^* & \ \ 89.62^* & \ \ 6.92^* \\
    Texturify & 4-RoSy Field & 31.08 & 1.75 & 59.55 & 4.97 \\
\midrule
    {\bf Ours} & 4-RoSy Implicit Field & {\bf 30.01} & {\bf 1.69} & {\bf 41.35} & {\bf 3.41} \\
\bottomrule
\end{tabular}
}
\caption{Evaluation on arbitrary texture generation, learned on real-world 2D images.
}
\label{tab:generation}
\end{table}

\begin{table}[tp]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Chairs} & \multicolumn{2}{c|}{Cars} & \multicolumn{2}{c|}{Chairs} & \multicolumn{2}{c}{Cars} \\
    & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c|}{ScanNet} & \multicolumn{2}{c}{CompCars} \\
\cmidrule{2-9}
    & \multicolumn{4}{c|}{Exact geometry} & \multicolumn{4}{c}{Close geometry} \\
\cmidrule{2-9}
    & FID & KID \times $10^2$ & FID & KID \times $10^2$ & FID & KID \times $10^2$ & FID & KID \times $10^2$ \\
\midrule
    EG3D & 146.6 & 9.49 & 297.9 & 20.82 & 318.8 & 27.39 & 334.4 & 36.96 \\
    Yu et al. & 153.1 & 10.2 & 289.4 & 18.88 & 329.8 & 28.60 & 367.2 & 41.24 \\
    GET3D & \ \ 265.6^* & \ \ 26.67^* & \ \ 248.8^* & \ \ 15.57^* & 336.5 & 38.74 & 282.6 & 31.67 \\
    Texturify & 155.9 & 10.94 & 301.4 & 20.63 & 342.2 & 33.65 & 354.3 & 39.61 \\
\midrule
    {\bf Ours} & {\bf 115.4} & {\bf 5.38} & {\bf 165.5} & {\bf 6.84} & {\bf 309.7} & {\bf 26.50} & {\bf 202.8} & {\bf 21.12} \\
\bottomrule
\end{tabular}
}
\caption{Evaluation on aligned queried texture generation on ShapeNet and ScanNet chairs, and CompCars cars, learned on real-world 2D images.
}
\label{tab:aligned-comp}
\end{table}

\begin{table}[tp]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Chairs} & \multicolumn{2}{c|}{Cars} & \multicolumn{2}{c|}{Chairs} & \multicolumn{2}{c}{Cars} \\
    & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c|}{ScanNet} & \multicolumn{2}{c}{CompCars} \\
\cmidrule{2-9}
    & \multicolumn{4}{c|}{Exact geometry} & \multicolumn{4}{c}{Close geometry} \\
\cmidrule{2-9}
    & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR \\
\midrule
    EG3D & 84.52 & 15.49 & 82.84 & 17.85 & 77.15 & 11.39 & 72.17 & 10.79 \\
    Yu et al. & 84.26 & 15.36 & 83.75 & 18.53 & 75.62 & {\bf 11.57} & 72.43 & 11.14 \\
    GET3D & 80.36 & 11.13 & 79.97 & 12.45 & 76.62 & 10.26 & {\bf 75.40} & {\bf 11.50} \\
    Texturify & 84.64 & {\bf 15.79} & {\bf 84.08} & {\bf 18.79} & 74.61 & 10.70 & 72.40 & 11.08 \\
\midrule
    {\bf Ours} & {\bf 85.62} & 15.32 & 84.04 & 17.95 & {\bf 78.86} & 11.35 & 72.76 & 11.07 \\
\bottomrule
\end{tabular}
}
\caption{Evaluation on aligned queried texture generation on ShapeNet and ScanNet chairs, and CompCars cars, learned on real-world 2D images.
}
\label{tab:aligned-comp-ssim-psnr}
\end{table}

\begin{table}[tp]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Chairs} & \multicolumn{2}{c|}{Cars} & \multicolumn{2}{c|}{Chairs} & \multicolumn{2}{c}{Cars} \\
    & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c|}{ScanNet} & \multicolumn{2}{c}{CompCars} \\
\cmidrule{2-9}
    & \multicolumn{4}{c|}{Exact geometry} & \multicolumn{4}{c}{Close geometry} \\
\cmidrule{2-9}
    & CLIP & LPIPS & CLIP & LPIPS & CLIP & LPIPS & CLIP & LPIPS \\
\midrule
    EG3D & 89.87 & 16.41 & 83.27 & 15.69 & 82.86 & 26.58 & 68.78 & 27.90 \\
    Yu et al. & 89.73 & 16.26 & 84.33 & 14.83 & 82.93 & 26.52 & 67.21 & 27.48 \\
    GET3D & 85.00 & 24.99 & 81.38 & 21.71 & 78.52 & 29.03 & 70.19 & {\bf 25.54} \\
    Texturify & 89.22 & 16.23 & 83.82 & {\bf 14.69} & 81.71 & 26.31 & 68.77 & 27.41 \\
\midrule
    {\bf Ours} & {\bf 92.27} & {\bf 14.64} & {\bf 85.91} & 14.77 & {\bf 84.28} & {\bf 25.64} & {\bf 77.96} & 27.32 \\
\bottomrule
\end{tabular}
}
\caption{Evaluation on aligned queried texture generation on ShapeNet and ScanNet chairs, and CompCars cars, learned on real-world 2D images.
}
\label{tab:aligned-comp-clip-lpips}
\end{table}

\begin{table}[tp]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Chairs} & \multicolumn{2}{c|}{Cars} & \multicolumn{2}{c|}{Chairs} & \multicolumn{2}{c}{Cars} \\
    & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c|}{ScanNet} & \multicolumn{2}{c}{CompCars} \\
\cmidrule{2-9}
    & \multicolumn{4}{c|}{Exact geometry} & \multicolumn{4}{c}{Close geometry} \\
\cmidrule{2-9}
    & FID & KID \times $10^2$ & FID & KID \times $10^2$ & FID & KID \times $10^2$ & FID & KID \times $10^2$ \\
\midrule
    EG3D & 155.2 & 9.13 & 326.8 & 24.48 & 319.4 & 27.18 & 352.3 & 39.15 \\
    Yu et al. & 160.0 & 9.88 & 343.3 & 32.71 & 327.1 & 28.20 & 385.4 & 51.37 \\
    GET3D & 271.9 & 26.54 & 254.4 & 16.63 & 337.3 & 38.76 & 264.7 & 29.23 \\
    Texturify & 174.2 & 11.74 & 344.2 & 25.34 & 333.3 & 28.81 & 376.8 & 42.33 \\
\midrule
    {\bf Ours} & {\bf 121.1} & {\bf 5.08} & {\bf 165.8} & {\bf 6.77} & {\bf 311.9} & {\bf 26.73} & {\bf 203.7} & {\bf 21.48} \\
\bottomrule
\end{tabular}
}
\caption{Evaluation on non-aligned queried texture generation on ShapeNet and ScanNet chairs, and ShapeNet and CompCars cars, learned on real-world 2D images.
}
\label{tab:non-aligned-comp}
\end{table}

\begin{table}[tp]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Chairs} & \multicolumn{2}{c|}{Cars} & \multicolumn{2}{c|}{Chairs} & \multicolumn{2}{c}{Cars} \\
    & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c|}{ScanNet} & \multicolumn{2}{c}{CompCars} \\
\cmidrule{2-9}
    & \multicolumn{4}{c|}{Exact geometry} & \multicolumn{4}{c}{Close geometry} \\
\cmidrule{2-9}
    & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR \\
\midrule
    EG3D & 83.69 & 15.26 & 82.30 & 17.13 & 76.24 & 11.07 & 72.33 & 10.90 \\
    Yu et al. & 83.18 & 15.23 & 78.44 & 12.31 & 75.09 & 11.44 & 72.16 & 10.94 \\
    GET3D & 79.49 & 11.00 & 80.28 & 12.31 & 76.79 & 10.44 & {\bf 75.29} & {\bf 11.46} \\
    Texturify & 83.37 & {\bf 15.46} & 82.89 & {\bf 17.81} & 74.26 & {\bf 11.56} & 72.22 & 10.99 \\
\midrule
    {\bf Ours} & {\bf 85.26} & 15.34 & {\bf 83.69} & 17.33 & {\bf 78.72} & 11.35 & 73.06 & 11.13 \\
\bottomrule
\end{tabular}
}
\caption{Evaluation on non-aligned queried texture generation on ShapeNet and ScanNet chairs, and ShapeNet and CompCars cars, learned on real-world 2D images.
}
\label{tab:non-aligned-comp-ssim-psnr}
\end{table}

\begin{table}[tp]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Chairs} & \multicolumn{2}{c|}{Cars} & \multicolumn{2}{c|}{Chairs} & \multicolumn{2}{c}{Cars} \\
    & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c|}{ScanNet} & \multicolumn{2}{c}{CompCars} \\
\cmidrule{2-9}
    & \multicolumn{4}{c|}{Exact geometry} & \multicolumn{4}{c}{Close geometry} \\
\cmidrule{2-9}
    & CLIP & LPIPS & CLIP & LPIPS & CLIP & LPIPS & CLIP & LPIPS \\
\midrule
    EG3D & 89.51 & 16.83 & 81.93 & 16.14 & 83.40 & 26.88 & 68.18 & 27.84 \\
    Yu et al. & 88.98 & 16.81 & 79.35 & 21.84 & 82.67 & 26.88 & 64.76 & 27.43 \\
    GET3D & 84.66 & 25.90 & 81.54 & 21.45 & 79.02 & 29.12 & 71.21 & {\bf 25.50} \\
    Texturify & 88.24 & 16.82 & 80.45 & 15.42 & 82.26 & 26.79 & 66.93 & 27.46 \\
\midrule
    {\bf Ours} & {\bf 91.57} & {\bf 14.96} & {\bf 85.42} & {\bf 14.97} & {\bf 84.28} & {\bf 25.72} & {\bf 77.71} & 27.36 \\
\bottomrule
\end{tabular}
}
\caption{Evaluation on non-aligned queried texture generation on ShapeNet and ScanNet chairs, and ShapeNet and CompCars cars, learned on real-world 2D images.
}
\label{tab:non-aligned-comp-clip-lpips}
\end{table}

\begin{table}[tp]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Chairs} & \multicolumn{2}{c|}{Cars} & \multicolumn{2}{c}{Chairs} \\
    & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c}{ScanNet} \\
\cmidrule{2-7}
    & \multicolumn{4}{c|}{Exact geometry} & \multicolumn{2}{c}{Close geometry} \\
\cmidrule{2-7}
    & FID & KID \times $10^2$ & FID & KID \times $10^2$ & FID & KID \times $10^2$ \\
\midrule
    EG3D & 297.4 & 28.53 & 343.6 & 26.57 & 355.2 & 33.31 \\
    Yu et al. & 303.4 & 29.10 & 351.1 & 26.75 & 362.6 & 34.20 \\
    GET3D & - & - & - & - & - & - \\
    Texturify & 307.9 & 29.63 & 357.1 & 27.05 & 370.4 & 34.85 \\
\midrule
    {\bf Ours} & {\bf 276.7} & {\bf 26.17} & {\bf 194.5} & {\bf 10.11} & {\bf 348.5} & {\bf 32.33} \\
\bottomrule
\end{tabular}
}
\caption{Evaluation on style transfer texture generation on ShapeNet and ScanNet chairs, and ShapeNet and CompCars cars, learned on real-world 2D images.
}
\label{tab:out-of-dom-comp}
\end{table}

\begin{table}[tp]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Chairs} & \multicolumn{2}{c|}{Cars} & \multicolumn{2}{c}{Chairs} \\
    & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c}{ScanNet} \\
\cmidrule{2-7}
    & \multicolumn{4}{c|}{Exact geometry} & \multicolumn{2}{c}{Close geometry} \\
\cmidrule{2-7}
    & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR \\
\midrule
    EG3D & 76.30 & 10.25 & 79.59 & 13.68 & 74.19 & 9.67 \\
    Yu et al. & 75.98 & {\bf 10.45} & 80.35 & 13.98 & 72.68 & {\bf 10.20} \\
    GET3D & - & - & - & - & - & - \\
    Texturify & 75.79 & 10.43 & 79.99 & 14.09 & 71.65 & 10.13 \\
\midrule
    {\bf Ours} & {\bf 77.48} & 9.99 & {\bf 80.96} & {\bf 14.17} & {\bf 76.55} & 9.96 \\
\bottomrule
\end{tabular}
}
\caption{Evaluation on style transfer texture generation on ShapeNet and ScanNet chairs, and ShapeNet and CompCars cars, learned on real-world 2D images.
}
\label{tab:out-of-dom-comp-ssim-psnr}
\end{table}

\begin{table}[tp]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Chairs} & \multicolumn{2}{c|}{Cars} & \multicolumn{2}{c}{Chairs} \\
    & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c}{ScanNet} \\
\cmidrule{2-7}
    & \multicolumn{4}{c|}{Exact geometry} & \multicolumn{2}{c}{Close geometry} \\
\cmidrule{2-7}
    & CLIP & LPIPS & CLIP & LPIPS & CLIP & LPIPS \\
\midrule
    EG3D & 81.62 & 27.77 & 80.72 & 20.18 & 81.54 & 29.98 \\
    Yu et al. & 81.31 & 27.48 & 78.69 & 19.68 & 81.21 & 29.77 \\
    GET3D & - & - & - & - & - & - \\
    Texturify & 80.70 & 27.43 & 78.59 & 19.67 & 80.99 & 29.65 \\
\midrule
    {\bf Ours} & {\bf 83.47} & {\bf 26.77} & {\bf 82.20} & {\bf 19.04} & {\bf 81.95} & {\bf 28.90} \\
\bottomrule
\end{tabular}
}
\caption{Evaluation on style transfer texture generation on ShapeNet and ScanNet chairs, and ShapeNet and CompCars cars, learned on real-world 2D images.
}
\label{tab:out-of-dom-comp-clip-lpips}
\end{table}

\begin{table}[tp]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Chairs (unaligned)} & \multicolumn{2}{c|}{Chairs (aligned)} & \multicolumn{2}{c}{Chairs (unaligned)} \\
    & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c|}{ScanNet} & \multicolumn{2}{c}{ScanNet} \\
\cmidrule{2-7}
    & FID & KID \times $10^2$ & FID & KID \times $10^2$ & FID & KID \times $10^2$ \\
\midrule
    w/o NOC & 124.3 & 5.53 & 312.4 & 26.79 & 314.8 & 27.36 \\
    w/o patches & 143.5 & 6.91 & 313.8 & 26.91 & 309.2 & 26.67 \\
    w/o surf. features & 127.1 & 5.80 & {\bf 306.7} & {\bf 26.45} & {\bf 308.5} & {\bf 26.55} \\
\midrule
    {\bf Ours} & {\bf 121.1} & {\bf 5.08} & 309.7 & 26.50 & 311.9 & 26.73 \\
\bottomrule
\end{tabular}
}
\caption{Evaluation on aligned queried texture generation on ShapeNet and ScanNet chairs, and CompCars cars, learned on real-world 2D images.
}
\label{tab:ablation}
\end{table}

\begin{table}[tp]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Chairs (unaligned)} & \multicolumn{2}{c|}{Chairs (aligned)} & \multicolumn{2}{c}{Chairs (unaligned)} \\
    & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c|}{ScanNet} & \multicolumn{2}{c}{ScanNet} \\
\cmidrule{2-7}
    & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR \\
\midrule
    w/o NOC & 84.87 & {\bf 15.73} & 77.79 & 11.27 & 77.99 & 11.43 \\
    w/o patches & 83.88 & 15.09 & 76.86 & {\bf 11.92} & 77.66 & {\bf 12.06} \\
    w/o surf. features & 85.15 & 15.36 & {\bf 79.02} & 11.48 & {\bf 79.05} & 11.52 \\
\midrule
    {\bf Ours} & {\bf 85.26} & 15.34 & 78.86 & 11.35 & 78.72 & 11.35 \\
\bottomrule
\end{tabular}
}
\caption{Evaluation on aligned queried texture generation on ShapeNet and ScanNet chairs, and CompCars cars, learned on real-world 2D images.
}
\label{tab:ablation-ssim-psnr}
\end{table}

\begin{table}[tp]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Chairs (unaligned)} & \multicolumn{2}{c|}{Chairs (aligned)} & \multicolumn{2}{c}{Chairs (unaligned)} \\
    & \multicolumn{2}{c|}{ShapeNet} & \multicolumn{2}{c|}{ScanNet} & \multicolumn{2}{c}{ScanNet} \\
\cmidrule{2-7}
    & CLIP & LPIPS & CLIP & LPIPS & CLIP & LPIPS \\
\midrule
    w/o NOC & 91.09 & 15.20 & 83.61 & 25.97 & 83.59 & 25.82 \\
    w/o patches & 89.68 & 16.27 & {\bf 85.09} & 25.82 & {\bf 84.97} & 25.86 \\
    w/o surf. features & 90.70 & 15.26 & 82.77 & {\bf 25.69} & 82.62 & {\bf 25.72} \\
\midrule
    {\bf Ours} & {\bf 91.57} & {\bf 14.96} & 84.36 & 25.72 & 84.28 & {\bf 25.72} \\
\bottomrule
\end{tabular}
}
\caption{Evaluation on aligned queried texture generation on ShapeNet and ScanNet chairs, and CompCars cars, learned on real-world 2D images.
}
\label{tab:ablation-clip-lpips}
\end{table}
